Read Cities through their Lines. Methodology to characterize spatial graphs

Cities can be seen as the epitome of complex systems. They arise from a set of interactions and components so diverse that is almost impossible to describe them exhaustively. Amid this diversity, we chose an object which orchestrates the development and use of an urban area : the road network. Following the established work on space syntax, we represent road networks as graphs. From this symbolic representation we can build a geographical object called the way. The way is defined by local rules independently from the direction in which the network is read. This complex object, and several indicators leaned upon it, allows us to carry out deep analysis of spatial networks, independent from their borders. With this methodology, we demonstrate how different road graphs, from various places in the world, show similar properties. We show how such analysis, based on the topological and topographical properties of their road networks, allows us to trace back some aspects of the historical and geographical contexts of city formation. We define a model of temporal differentiation, where the structural changes through time in the network are highlighted. This methodology was thought to be generic so it can be used with several kinds of spatial networks, opening the panel of research applications and future work. Key words : Road network, Graph theory, Spatial analysis, Complex system, Urban modelling.

==> annexes/A2_3_panel_cartes.tex <==
\FloatBarrier 
\chapter{Panel}\label{ann:chap_panel}



\section{Graphes viaires (villes)}\label{ann:sec_panel_viaireville}

\clearpage

\FloatBarrier
\subsection{Paris}

\begin{figure}[h]
	\centering
	\begin{subfigure}[t]{0.8\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{images/cities/paris_0_brut.pdf}
	    \caption*{Graphe brut}
	\end{subfigure}
	\begin{subfigure}[t]{0.8\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{images/cities/paris_2_degre.pdf}
	    \caption*{Degrés des voies}
	\end{subfigure}
\end{figure}

\begin{figure}[h]
	\centering
	\begin{subfigure}[t]{0.8\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{images/cities/paris_3_closeness.pdf}
	    \caption*{Closeness des voies}
	\end{subfigure}
	\begin{subfigure}[t]{0.8\textwidth}
	    \centering
	    \includegraphics[width=\textwidth]{images/cities/paris_4_ortho.pdf}
	    \caption*{Orthogonalité des voies}
	\end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Avignon}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/avignon_large_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/avignon_large_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/avignon_large_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/avignon_large_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Bordeaux}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/bordeaux_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/bordeaux_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/bordeaux_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/bordeaux_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Brive}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/brive_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/brive_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/brive_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/brive_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Cergy-Pontoise}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/cergy_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/cergy_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/cergy_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/cergy_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Villers-sur-Mer}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/villers_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/villers_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/villers_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/villers_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Bruxelles}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/bruxelles_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/bruxelles_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/bruxelles_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/bruxelles_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Londres}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/londres_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/londres_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/londres_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/londres_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Barcelone}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/barcelone_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/barcelone_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/barcelone_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/barcelone_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Rotterdam}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/rotterdam_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/rotterdam_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/rotterdam_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/rotterdam_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Manhattan}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/manhattan_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/manhattan_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/manhattan_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/manhattan_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{San-Francisco}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/sanfrancisco_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/sanfrancisco_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/sanfrancisco_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/sanfrancisco_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Santa-Fe}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/santafe_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/santafe_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/santafe_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/santafe_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Manaus}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/manaus_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/manaus_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/manaus_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/manaus_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Cuzco}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/cuzco_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/cuzco_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/cuzco_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/cuzco_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Téhéran}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/teheran_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/teheran_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/teheran_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/teheran_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Varanasi}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/varanasi_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/varanasi_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/varanasi_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/varanasi_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Kyoto}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        %\includegraphics[width=\textwidth]{images/cities/kyoto_0_brut.pdf}
        \includegraphics[width=\textwidth]{images/cities/kyoto_2_degre.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/kyoto_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/kyoto_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/kyoto_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Casablanca}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/casablanca_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/casablanca_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/casablanca_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/casablanca_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Nairobi}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nairobi_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nairobi_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nairobi_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nairobi_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\section{Graphes viaires (quartiers)}\label{ann:sec_panel_viairequart}

\clearpage

\subsection{Neuf-Brisach}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/brisach_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/brisach_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/brisach_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/brisach_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Cucq}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/cucq_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/cucq_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/cucq_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/cucq_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Lille}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/lille_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/lille_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/lille_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/lille_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Vitry-le-François}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/vitry_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/vitry_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/vitry_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/vitry_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier


\subsection{La Roche-sur-Yon}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/yon_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/yon_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/yon_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/quartiers/yon_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier


\section{Graphes artificiels}\label{ann:sec_panel_artifi}

\clearpage


\subsection{Bruit faible}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/reseaux_artificiels/bruitfaible_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/reseaux_artificiels/bruitfaible_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/reseaux_artificiels/bruitfaible_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
%    \begin{subfigure}[t]{0.8\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{images/cities/reseaux_artificiels/bruitfaible_4_ortho.pdf}
%        \caption*{Orthogonalité des voies}
%    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Bruit fort}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/reseaux_artificiels/bruitfort_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/reseaux_artificiels/bruitfort_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/reseaux_artificiels/bruitfort_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/reseaux_artificiels/bruitfort_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Avec générations}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/reseaux_artificiels/generation_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/reseaux_artificiels/generation_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/reseaux_artificiels/generation_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/reseaux_artificiels/generation_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Avec angles}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/reseaux_artificiels/angles_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/reseaux_artificiels/angles_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/reseaux_artificiels/angles_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/reseaux_artificiels/angles_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier


\section{Graphes de craquelures}\label{ann:sec_panel_craqs}

\clearpage

\subsection{argile 1}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nature/craq1_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nature/craq1_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nature/craq1_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nature/craq1_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{argile 2}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nature/craq2_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nature/craq2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nature/craq2_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nature/craq2_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier



\section{Graphes biologiques}\label{ann:sec_panel_biol}

\clearpage

\subsection{feuille}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nature/feuille1_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nature/feuille1_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nature/feuille1_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nature/feuille1_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{gorgone}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nature/gorgone1s_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nature/gorgone1s_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nature/gorgone1s_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/nature/gorgone1s_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier


\section{Graphes hydrographiques}\label{ann:sec_panel_hydro}

\clearpage

\subsection{Amazonie}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/waterways/amazonie_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/waterways/amazonie_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/waterways/amazonie_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/waterways/amazonie_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Italie (Nord)}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/waterways/norditalie_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/waterways/norditalie_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/waterways/norditalie_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/waterways/norditalie_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier


\subsection{Inde (Sud)}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/waterways/sudinde_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/waterways/sudinde_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/waterways/sudinde_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/waterways/sudinde_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\section{Graphes ferrés}\label{ann:sec_panel_ferre}

\clearpage

\subsection{Belgique}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/railways/belgique_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/railways/belgique_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/railways/belgique_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/railways/belgique_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier


\subsection{Californie}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/railways/californie_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/railways/californie_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/railways/californie_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/railways/californie_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier

\subsection{Russie}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/railways/russie_0_brut.pdf}
        \caption*{Graphe brut}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/railways/russie_2_degre.pdf}
        \caption*{Degrés des voies}
    \end{subfigure}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/railways/russie_3_closeness.pdf}
        \caption*{Closeness des voies}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cities/railways/russie_4_ortho.pdf}
        \caption*{Orthogonalité des voies}
    \end{subfigure}
\end{figure}

\FloatBarrier





==> annexes/A2_4_diachronie_tab_PEUTETRE.tex <==
 
\section{Détail statistique des variations relatives}\label{ann:sec_dia_stats}

\subsection{Avignon}

\begin{table}
\begin{center}

\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline

période & $N_{arcs(modifiés)}$ & $\overline{\Delta_{relatif}}$ & $\sigma(\Delta_{relatif})$  & $max \vert \Delta_{relatif}\vert$ & $\sum \vert \Delta_{relatif} \vert$ & $\sum_{\Delta_{relatif}<0} \vert \Delta_{relatif} \vert$ & $\sum_{\Delta_{relatif}>0} \vert \Delta_{relatif} \vert$ \\ \hline

1760 - 1819 & 72 & -0.0502 & 0.0583 & 0.3644 & 51.87 & -51.41 & 0.46   \\ \hline
1819 - 1836 & 54 & 0.0007 & 0.0302 & 0.4569 & 5.18 & -2.23 & 2.94 \\ \hline
1836 - 1854 & 112 & 0.0552 & 0.1055 & 0.4999 & 80.96 & -11.16 & 69.79 \\ \hline
1854 - 1879 & 80 & -0.0145 & 0.0672 & 0.3473 & 35.99 & -25.95 & 10.05 \\ \hline
1879 - 1910 & 51 & -0.0130 & 0.0886 & 0.9611 & 49.05 & -31.84 & 17.21 \\ \hline
1910 - 1926 & 77 & 0.0105 & 0.0430 & 0.4514 & 21.76 & -5.03 & 16.73 \\ \hline
1926 - 1959 & 41 & 0.0250 & 0.0415 & 0.3301 & 30.19 & -1.01 & 29.19 \\ \hline
1959 - 1970 & 40 & -0.0101 & 0.0683 & 0.5273 & 33.73 & -22.58 & 11.15 \\ \hline
1970 - 2014 & 91 & 0.0509 & 0.0673 & 0.3980 & 67.59 & -5.18 & 62.41 \\ \hline

\end{tabular}
\end{center}
\caption{Détail statistique des variations relatives $\Delta_{relatif}$ pour chaque période d'étude du centre d'Avignon.}
\label{tab:avignon_delta2}
\end{table}


\subsection{Rotterdam}


\begin{table}
\begin{center}

\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline

période & $N_{arcs(modifiés)}$ & $\overline{\Delta_{relatif}}$ & $\sigma(\Delta_{relatif})$  & $max \vert \Delta_{relatif}\vert$ & $\sum \vert \Delta_{relatif} \vert$ & $\sum_{\Delta_{relatif}<0} \vert \Delta_{relatif} \vert$ & $\sum_{\Delta_{relatif}>0} \vert \Delta_{relatif} \vert$ \\ \hline

\multicolumn{6}{|c|}{Réseau entier}   \\ \hline

1374 - 1570 & 651 & -0.0567 & 0.1212 & 0.7662 & 139.44 & -107.29 & 32.15  \\ \hline
1570 - 1600 & 426 & -0.0546 & 0.1241 & 0.9404 & 185.12 & -143.00 & 42.12  \\ \hline
1600 - 1625 & 287 & 0.0911 & 0.0941 & 0.3907 & 207.92 & -6.59 & 201.32  \\ \hline
1625 - 1890 & 1809 & -0.0491 & 0.0617 & 0.2872 & 125.31 & -113.06 & 12.26  \\ \hline
1890 - 1907 & 1140 & -0.0433 & 0.0521 & 0.3144 & 159.27 & -153.94 & 5.33  \\ \hline
1907 - 1920 & 1348 & 0.04467 & 0.0567 & 0.2971 & 215.63 & -14.94 & 200.69  \\ \hline
1920 - 1940 & 2891 & 0.0543 & 0.0710 & 0.6344 & 315.22 & -28.94 & 286.28  \\ \hline
1940 - 1955 & 3482 & -0.0498 & 0.0909 & 0.7473 & 476.04 & -389.15 & 86.89  \\ \hline

\multicolumn{6}{|c|}{Réseau découpé} \\ \hline

1374 - 1570 & 417 & 0.0192 & 0.1190 & 0.7506 & 78.58 & -30.10 & 48.49 \\ \hline
1570 - 1600 & 230 & -0.1005 & 0.1071 & 0.9503 & 163.86 & -148.78 & 15.08 \\ \hline
1600 - 1625 & 287  & 0.1158 & 0.1140 & 0.3927 & 187.34 & -6.61 & 180.73 \\ \hline
1625 - 1890 & 1449 & -0.0793 & 0.0616 & 0.4893 & 131.23 & -127.16 & 4.08 \\ \hline
1890 - 1907 & 1059 & -0.0271 & 0.0495 & 0.2761 & 93.98 & -83.53 & 10.45 \\ \hline
1907 - 1920 & 1059 & 0.0327 & 0.0508 & 0.3337 & 137.87 & -13.41 & 124.45 \\ \hline
1920 - 1940 & 2251 & 0.0131 & 0.0625 & 0.6588 & 155.12 & -51.74 & 103.36 \\ \hline
1940 - 1955 & 3105 & 0.0120 & 0.0998 & 0.7344 & 335.15 & -138.62 & 196.53 \\ \hline

\end{tabular}
\end{center}
\caption{Détail statistique des variations relatives $\Delta_{relatif}$ pour chaque période d'étude du nord de Rotterdam (entier et redécoupé).}
\label{tab:rott_delta2}
\end{table}

==> couverture2_old.tex <==

%%%%%%%%%% COUVERTURE

\pagestyle{empty}

\begin{titlepage}

	\newgeometry{left=0cm,right=0cm,top=0cm}

	\AddToShipoutPicture*{
		\put(0,0){%
		\parbox[b][\paperheight]{\paperwidth}{%
		\vfill
		\centering
		\includegraphics[width=\paperwidth,height=\paperheight]{images/couverture/couv2_retouch.png}%
		\vfill
		}}	
	} 
	
	\flushleft
	
	\vspace*{10.8cm}
	
	\fcolorbox{white}{white}{

	\begin{minipage}{4cm}
		\centering
		\includegraphics[width=75pt]{images/couverture/Logo_P7.pdf}
	\end{minipage} \hfill
	\begin{minipage}{14cm}
		\sffamily
		\centering
		\vspace{1cm}
		
		{\Large Thèse de doctorat - spécialité Physique}
		
		\vspace{1cm}	
			
		{\Huge \textbf{Lire les Lignes de la Ville}}
		
		\vspace{0.5cm}	
			
		{\LARGE \textbf{Méthodologie de caractérisation des graphes spatiaux}}
		
		\vspace{1cm}
		
		{\huge Claire Lagesse}
		
		\vspace{1cm}
	
	\end{minipage} \hfill
	\begin{minipage}{5cm}
		\hspace{1cm}
	\end{minipage}	

	}
	
	\vfill % Fill the rest of the page with whitespace
	
	\restoregeometry

\end{titlepage}

%%%%%%%%%% PAGE DE GARDE

\begin{titlepage}

	\sffamily

	\newgeometry{left=1cm,right=1cm,top=1cm, bottom=0cm}

	\center
	
	% En-tête
	\begin{minipage}{\textwidth}
		\centering
		Université Paris-Diderot (Paris 7) Sorbonne Paris Cité
	\end{minipage}
	\hrule
	\begin{minipage}{0.45\textwidth}
		\flushleft
		UFR de physique
	\end{minipage}	\hfill
	\begin{minipage}{0.45\textwidth}
		\flushright
		École Doctorale 564 Physique en Île-de-France
	\end{minipage}
		
	\vspace*{3cm}

	% Auteur
	\begin{minipage}{12cm}
		\centering
		
		{\huge Claire LAGESSE}		
		
		\vspace{0.5cm}
		\vspace{2cm}			
		{\large a présenté publiquement le 25 septembre 2015 ses travaux pour l'obtention du}
		
		\vspace{0.5cm}	
		
		{\LARGE titre de docteur - spécialité Physique}
	\end{minipage}
	
	\vspace*{2cm}
	
	% Titre
	\begin{minipage}{12cm}
		\centering
			
		{\LARGE Lire les Lignes de la Ville}
		
		\vspace{0.5cm}	
			
		{\Large Méthodologie de caractérisation des graphes spatiaux}
	
	\end{minipage}
	
		
	\vspace*{4cm}

	% Jury
	\begin{minipage}{8cm}
		\begin{center}

\renewcommand{\arraystretch}{0.5}		
		{\Large
		
		\begin{tabular}{l l}
			%Président & Bidule \\
			Directeur & Stéphane DOUADY \\
			Co-directrice & Patricia BORDIN \\
			Rapporteurs & Arnaud BANOS \\
			 & Alain BARRAT \\
			Examinateurs & Claude GRASLAND \\
			 & Jean-Loup GUILLAUME \\
			 & Renaud LAMBIOTTE \\
			 & Jacynthe POULIOT \\
		\end{tabular}				
		
		}
		
		\end{center}
	\end{minipage}
		
	\vspace*{2cm}
	
	% Pied de page
	\hrule
	\begin{minipage}[t]{3cm}
		\centering
		\includegraphics[width=0.5\textwidth]{images/couverture/Logo_MSC.pdf}
		
		Laboratoire Matière et Systèmes Complexes
	\end{minipage} \hspace*{0.5cm} \hfill
	\begin{minipage}[t]{3cm}
		\centering
		\includegraphics[width=0.5\textwidth]{images/couverture/Logo_CNRS.pdf}
		
		Centre Nationale de le Recherche Scientifique		
	\end{minipage} \hspace*{0.5cm} \hfill
	\begin{minipage}[t]{3cm}
		\centering
		\includegraphics[width=0.5\textwidth]{images/couverture/Logo_ANR.jpg}
		
		Agence Nationale de la Recherche
	\end{minipage} \hspace*{0.5cm} \hfill
	\begin{minipage}[t]{3cm}
		\centering
		\includegraphics[width=0.5\textwidth]{images/couverture/Logo_ESTP.jpg}
		
		École Spéciale des Travaux Publics
	\end{minipage} \hspace*{0.5cm} \hfill
	\begin{minipage}[t]{3cm}
		\centering
		\includegraphics[width=0.5\textwidth]{images/couverture/Logo_IRC.png}
		
		Institut de Recherche en Constructibilité
	\end{minipage}
	
	
	

%	\vfill % Fill the rest of the page with whitespace
	
	\restoregeometry

\end{titlepage}

\pagestyle{fancy}


==> formules.tex <==
%\begin{equation}
%orthogonalite(v_{ref}) = \frac {\sum\limits^{}_{s \in v_{ref}} \  \sum\limits^{}_{arc_i \cap s \wedge arc_i \notin v_{ref}} \  \min(\sin(\varphi_{arc_i arc_j})) / (arc_j \cap s \wedge arc_j \in v_{ref})}{connectivite(v_{ref}
%)}
%\label{eq:orthogonalite}
%\end{equation}


\begin{equation}
betweenness(v_{ref})= \sum_{v_1 \neq v_2 \neq v_{ref} \in G}\frac{\sigma_{v_1v_2}(v_{ref})}{\sigma_{v_1v_2}}
\label{eq:betw_voies}
\end{equation}

\begin{equation}
betweenness(a_{ref})= \sum_{a_1 \neq a_2 \neq a_{ref} \in G}\frac{\sigma_{a_1a_2}(a_{ref})}{\sigma_{a_1a_2}}
\label{eq:betw_arcs}
\end{equation}


\begin{equation}
utilisation(v_{ref})= \sum_{v_1 \neq v_2 \neq v_{ref} \in G}\sigma_{v_1v_2}(v_{ref})
\label{eq:ut_sommets}
\end{equation}

\begin{equation}
utilisation(a_{ref})= \sum_{a_1 \neq a_2 \neq a_{ref} \in G}\sigma_{a_1a_2}(a_{ref})
\label{eq:ut_arcs}
\end{equation}

\begin{equation}
closeness(v_{ref})=\frac{1}{\sum_{v \in G} d_{simple}(v,v_{ref})}
\label{eq:closeness_voies}
\end{equation}


\begin{equation}
closeness(a_{ref})=\frac{1}{\sum_{a \in G} d_{simple}(a,a_{ref})}
\label{eq:closeness_arcs}
\end{equation}

\begin{equation}
  \Delta_{relatif}(a_{ref}) = (-1) \times \frac{\Delta access(a_{ref})}{accessibilite_{G_2}(a_{ref})}
\label{eq:deltafin}
\end{equation}

\begin{equation}
  \Delta_{brut}(a_{ref}) = (-1) \times \frac{\Delta_{brut} access(a_{ref})}{accessibilite_{G_2}(a_{ref})}
\label{eq:deltafin}
\end{equation}


\begin{equation}
\delta_{ajouts}(a_{ref}) = \sum_{a_{aj} \in G_2} (d_{simple}(a_{ref}, a_{aj}) \times longueur(a_{aj}))
\label{eq:deltaadd}
\end{equation}

\begin{equation}
\delta_{suppressions}(a_{ref}) = \sum_{a_{sup} \in G_1} (d_{simple}(a_{ref}, a_{sup}) \times longueur(a_{sup}))
\label{eq:deltarem}
\end{equation}

\begin{equation}
\Delta access(a_{ref}) = \Delta _{brut}access(a_{ref}) -  \delta_{ajouts}(a_{ref}) + \delta_{suppressions}(a_{ref})
\label{eq:deltaccess}
\end{equation}

\begin{eqnarray*}
  \Delta access(a_{ref}) &=& (accessibilite{G_2}(a_{ref}) - \delta_{ajouts}(a_{ref})) \\
  & & - (accessibilite{G_1}(a_{ref}) - \delta_{suppressions}(a_{ref})) \\
  &=& \Delta _{brut}access(a_{ref}) -  \delta_{ajouts}(a_{ref}) + \delta_{suppressions}(a_{ref})
\label{eq:deltatot}
\end{eqnarray*}

\begin{equation}
accessibilite(v_{ref})=\sum_{a_{ref} \in v_{ref}} [d_{simple}(a,a_{ref}) \times longueur(a)]
\label{eq:access}
\end{equation} 


==> guide_de_lecture/formules.tex <==
%% LOCAL

%PRIMAIRE

\begin{equation}
 degre(v_{ref}) = Card(v \in G / v \cap v_{ref})
 \label{eq:degre}
\end{equation}

\begin{equation}
 connectivite(v_{ref}) = \sum_{s \in v_{ref}} Card(a / [(s \in a) \wedge (a \notin v_{ref})])
 \label{eq:connectivite}
\end{equation}

%SECONDAIRE

\begin{equation}
 degreDesserte(v_{ref}) = connectivite(v_{ref}) - degre(v_{ref})
 \label{eq:degDesserte}
\end{equation}

\begin{equation}
espacement(v_{ref}) = \frac {longueur(v_{ref})}{connectivite(v_{ref})}
\label{eq:espacement}
\end{equation}

\begin{equation}
orthogonalite(v_{ref}) = \frac {\sum_{s \in v_{ref}} \sum_{arc_i \cap s \wedge arc_i \notin v_{ref}} \min(\sin(\theta_{arc_i arc_j})) / (arc_j \cap s \wedge arc_j \in v_{ref})}{connectivite(v_{ref})}
\label{eq:orthogonalite}
\end{equation}

%%GLOBAL

%PRIMAIRE

\begin{equation}
closeness(v_{ref})=\frac{1}{\sum_{v \in G} d_{simple}(v,v_{ref})}
\label{eq:clo}
\end{equation}

%SECONDAIRE

\begin{equation}
accessibiliteMaillee(v_{ref})= closeness(v_{ref}) \times orthogonalite(v_{ref})
\label{eq:accessmail}
\end{equation} 


==> pensesy.tex <==

Sur Avignon, ville européenne moyenâgeuse, nous observons que cet indicateur combiné appliqué aux voies est caractéristique des structures les plus anciennes autour du centre ville : centrales et maillées. L'autoroute apparaît également comme fort accessible car les voies qui la coupent perpendiculairement sans y être liées sont considérées comme connectées. C'est donc un artefact lié aux données. Les voies récentes de contournement du centre ville sont, elles, bien classées avec une accessibilité maillée faible. Nous reviendrons sur les limites de notre approche en deuxième partie, dont le cas de l'autoroute est une illustration ici. 

\FloatBarrier
\subsection{Bordeaux Rive Droite}

La rive droite de Bordeaux a été formée par l'effondrement de la falaise dans le fleuve, donnant naissance à l'île de Mayorgue. La progression de la Garonne suite à cet événement a déplacé la rive droite du fleuve, laissant un espace où il était possible de réaliser des constructions. Le parcellaire irrégulier sur cette partie en conserve la mémoire. Sa forme est rendue intelligible par le scénario de construction du paysage. 
 

 
 
 
Matrice d'adjacence



Poids : Les valeurs \enquote{1} de la matrice d'adjacence sont donc transformées pour faire apparaître des valeurs pondérées qui seront prises en compte lors du calcul.

FAIRE UN EXEMPLE DE MATRICE D’ADJACENCE

Afin de déterminer quels sont les arcs les plus centraux, nous utilisons le \textit{line graph} de notre graphe spatial.  Dans celui-ci, chaque sommet représente un arc. Un lien sera créé entre deux sommets du \textit{line graph} si les deux arcs correspondant s'intersectent dans le graphe primal. A partir de ce \textit{line graph}, nous construisons la matrice d'adjacence. La pondération de celle-ci, pour chaque intersection de sommets (correspondant à des arcs) sera faite avec une combinaison linéaire des longueurs des arcs du graphe primal s'intersectant. Ainsi, si deux arcs $arc_i$ et $arc_j$ s'intersectent à un sommet $s$, $M(arc_i,arc_j) = longueur(arc_i) + longueur(arc_j)$. Ainsi, si l'on considère le chemin entre les deux arcs grâce à la matrice d'adjacence, on se rend compte que toutes les longueurs sont comptées deux fois sauf celle de l'arc initial et celle de l'arc final, ce qui exacerbe le poids des arcs longs et favorise ainsi les chemins utilisant des petits arcs.




Manhattan et ses alentours dont les connexions entre îles apportent une configuration supplémentaire. Nous nous sommes penchés sur la généralisation d'un réseau de craquelures, car la vectorisation de ce type de réseaux est bruitée et nécessite un post-traitement.






==> resume_couv.tex <==
%--------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------
\clearpage{\pagestyle{empty}\cleardoublepage}
\pagestyle{empty}

~\newpage

\changepage{20mm}{10mm}{-5mm}{-5mm}{}{-5mm}{-5mm}{}{}
\paragraph{Résumé}

\

couv en francais

\vspace{1cm}

\paragraph{Abstract}

\

couv in english 
%--------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------


